IT$^3$: Idempotent Test-Time Training

Deep learning models often struggle when deployed in real-world settings due to distribution shifts between training and test data. While existing approaches like domain adaptation and test-time training (TTT) offer partial solutions, they typically require additional data or domain-specific auxiliary tasks. We present Idempotent Test-Time Training (IT$^3$), a novel approach that enables on-the-fly adaptation to distribution shifts using only the current test instance, without any auxiliary task design. Our key insight is that enforcing idempotence -- where repeated applications of a function yield the same result -- can effectively replace domain-specific auxiliary tasks used in previous TTT methods. We theoretically connect idempotence to prediction confidence and demonstrate that minimizing the distance between successive applications of our model during inference leads to improved out-of-distribution performance. Extensive experiments across diverse domains (including image classification, aerodynamics prediction, and aerial segmentation) and architectures (MLPs, CNNs, GNNs) show that IT$^3$ consistently outperforms existing approaches while being simpler and more widely applicable. Our results suggest that idempotence provides a universal principle for test-time adaptation that generalizes across domains and architectures.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> fig/related_viz.tex <==
\begin{figure}[ht!]
    \centering
    \begin{minipage}{.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ign_idea.jpg}
        \caption{\small {\bf Idempotent Generative Networks (IGN) idea.} visualization for IGN idea}
        \label{fig: airfoils}
    \end{minipage}%
    \hfill%
    \begin{minipage}{.59\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/zigzag_teaser.pdf}
        \caption{\small {\bf Zigzag idea.} visualization for zigzag idea}
        \label{fig:sampling}
    \end{minipage}
\end{figure}

==> fig/roads_iters.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
 % \vspace{-2mm}
    \includegraphics[width=0.99\textwidth]{images/roads_iters/roads_iters_1.pdf} \\
    \includegraphics[width=0.99\textwidth]{images/roads_iters/roads_iters_2.pdf} \\
    \includegraphics[width=0.99\textwidth]{images/roads_iters/roads_iters_4.pdf} \\
    \includegraphics[width=0.99\textwidth]{images/roads_iters/roads_iters_5.pdf} \\
    \includegraphics[width=0.99\textwidth]{images/roads_iters/roads_iters_6.pdf}
    \centering
     \vspace{-6mm}
    \caption{\small {\bf Additional qualitative results of \itt{} on Road Segmentation.} From left to right: (1) Original aerial image, (2) Not optimized output, (3) \itt{} output at the 5th iteration, (4) \itt{} output at the 15th iteration, and (5) Ground truth label. The segmentation quality improves significantly with \itt{} iterations, as observed in the progressively refined outputs at the 5th and 15th iterations.}

    % \vspace{-5mm}
    \label{fig:zigzag}
\end{figure}

==> fig/roads_task2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \begin{minipage}{.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/road_ims2.pdf}
        \vspace{-7mm}
        \caption{\small {\bf Road Samples.} 
        RoadTracer train dataset \textbf{(left)} includes urban areas of cities in US. From RoadTracer test dataset, we selected images of cities that are not included in train dataset as OOD samples \textbf{(right)}.
        }
        \label{fig:roads_ims2}

        \vspace{2mm}

        \includegraphics[width=\textwidth]{images/roads_mean-2.pdf}
        \vspace{-7mm}
        \caption{\small {\bf Roads mean quality score on OOD images.} The plot compares \itt{} to the vanilla model, showing better performance retention as data shifts from the training distribution.}
        \label{fig:roads_mean_results2}
        
    \end{minipage}%
    \hfill%
    \begin{minipage}{.56\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/roads_box-2.pdf}
        \vspace{1mm}
        \caption{\small {\bf Roads results on OOD images.} \textcolor[HTML]{96cac1}{\textbf{Not optimized}} corresponds to a single model without TTT applied. \itt{} with [\textcolor[HTML]{FFDAB9}{\textbf{batch=4}}, \textcolor[HTML]{C1BED6}{\textbf{batch=8}}, and \textcolor[HTML]{EA8E83}{\textbf{batch=16}}] represents our method at different batch sizes. As the data shifts further from the training distribution, our method degrades less, with larger batches preserving performance more effectively.}
        \label{fig:roads_box_results2}
    \end{minipage}
\end{figure}


==> fig/teaser.tex <==
\begin{figure}[ht!]
 % \vspace{-2mm}
    \includegraphics[width=0.99\textwidth]{images/ittt_teaser.pdf}
    \centering
    \vspace{-4mm}
    \caption{\small {\bf Idempotent test-time training framework.} During inference, the model receives an input \( x \) with an initial signal (empty or corrupted). It makes two sequential predictions: \( \hat{M}(x, 0) \) for the empty signal and \( \hat{M}(x, y_0) \) for the given signal. The difference between these outputs defines the idempotence loss, used in the test-time optimization step. This process allows the model to adapt to corrupted and OOD data, improving robustness during inference. \ND{blueprint for the teaser image} \ND{fix latex on the plot}} 
    \vspace{-2mm}
    \label{fig:zigzag}
\end{figure}


==> tex/idem_to_ood.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{From Idempotence to OOD generalization}


\textbf{(1) When training with the ZigZag approach, discrepancy between recursive calls of the model, $\| y_1 - y_0 \|$, measures the extent to which an input is out-of-distribution (OOD):}
In the ZigZag work (Durasov et al.) a model is modified to accept an additional input (either the true label or a “don’t know” signal) when training. At test time, the network is applied recursively twice. First computing $y_0 = f(x,0)$, and then $y_1 = f(x,y_0)$. The ZigZag paper empirically shows a measure for prediction uncertainty: 
 d=\| y_1 - y_0 \|$

The logic is that if $y_0$ approximates the true label $y$, then when the network is fed the pair $(x,y_0)$ (a valid input as per training), it returns a prediction $y_1$ such that $y_0 \approx y_1$, and thus $d$ is small. On the other hand, if $y_0$ is far from $y$, feeding the pair $(x, y_0)$ to the network amounts to giving it an input that is OOD w.r.t. the data distribution it was trained on. In such a case, the result $y_1$ becomes unpredictable, somewhat random, and is unlikely to be close to $y_0$. In other words, just like $(x,0)$ is OOD if $x$ is OOD, so is $(x,y_0)$ OOD and then it is not mapped to its $y$ argument, like a valid in-distribution $(x,y_0)$ pair would. For further details see Durasov et al.

\textbf{We can use $\| y_1 - y_0 \|$ as a loss, and reduce 'OODness':}
If we know how to measure the extent to which an input is OOD, why not actively update the model to reduce this value, so that this input is now on distribution? Based on the TTT approach, we apply a short input-specific training session to reduce $L_{\mathrm{IT^3}} =\| y_1 - y_0 \|$.

\textbf{(3) But what are we optimizing? Distance from idempotence!:}
Let us now expand the expression: 
$$L_{\mathrm{IT^3}} = \| y_1 - y_0 \| = \| f(x, f(x,0)) - f(x,0) \|.$$ Examining the model $f$, we see that if $L_{\mathrm{IT^3}}=0$, then the function $f(x,\cdot)$ is idempotent for that particular $x$ with respect to its second argument $y_0$. This essentially means that the degree to which $f(x,\cdot)$ deviates from idempotence given a certain $x$ is a proxy to how likely it is for that $x$ to be on the training data distribution and an $(x,y_0)$ valid pair should be invariant to $f$. The TTT session minimizes exactly that distance.

\textbf{(4) Can we directly minimize the distance from idempotence?:}
Minimizing the idempotence loss is not trivial.  Naively doing so can lead to pitfalls such as reinforcing erroneous predictions.  However this is done in the IGN paper. IGN highlights that minimizing the idempotence loss induces two gradient pathways: one that drives $f(x,0)$ toward the correct manifold (desirable) and another that may cause the manifold to expand so it includes  $f(x,0)$ (undesirable). To counteract this, IGN introduces a “tightness objective” that effectively limits the expansion by selectively updating the appropriate pathway.

\textbf{(5) Optimizing for Idempotence in IT$^3$:}
Following a similar rationale, our method avoids passing gradients through the second application of $f$. Instead, we use a frozen copy of the network (or update it via an exponential moving average) when computing the second prediction.
The core intuition is that we do not want $y_1$ to be drawn toward a flawed $y_0$. Rather, we want to adjust the function $f(x,\cdot)$ so that, for a given input $x$, the prediction $y_0$ is refined so that the subsequent prediction $y_1=f(x,y_0)$ remains close to $y_0

\textbf{(6) Projection onto distribution perspective:}
Finally, as discussed in Appendix B, this idempotence condition can be interpreted as projecting the $(x,y)$ pair onto the manifold of valid in-distribution examples. In other words, enforcing idempotence generalizes the concept of an orthogonal projection (where $P^2=P$) to our non-linear setting. For a more detailed derivation and discussion of this projection perspective, we refer the reviewer to Appendix B.
